SharedRep-RLHF: A Shared Representation Approach to RLHF with Diverse Preferences

Uniform-reward reinforcement learning from human feedback (RLHF), which trains a single reward model to represent the preferences of all annotators, fails to capture the diversity of opinions across sub-populations, inadvertently favoring dominant groups. The state-of-the-art, MaxMin-RLHF, addresses this by learning group-specific reward models, and by optimizing for the group receiving the minimum reward, thereby promoting fairness. However, we identify that a key limitation of MaxMin-RLHF is its poor performance when the minimum-reward group is a minority. To mitigate this drawback, we introduce a novel framework, termed {\em SharedRep-RLHF}. At its core, SharedRep-RLHF learns and leverages {\em shared traits} in annotations among various groups, in contrast to learning separate reward models across groups. We first show that MaxMin-RLHF is provably suboptimal in learning shared traits, and then quantify the sample complexity of SharedRep-RLHF. Experiments across diverse natural language tasks showcase the effectiveness of SharedRep-RLHF compared to MaxMin-RLHF with a gain of up to 20% in win rate.

==> figures/ablation/ablation_plot.tex <==
\pgfplotsset{scaled x ticks=false}

\begin{tikzpicture}
    \begin{axis}[
        %enlargelimits=false,
        title=Ablation,
        xlabel=Inner Dimension $k$,
        ylabel=\texttt{Shared-Pref} $\pi_{\rm PPO}$ Avg. Score,
        symbolic x coords={2,4,16,32},
        legend pos=south east,
        ymajorgrids=true,
        xmajorgrids=true,
        grid style=dotted,
        height=5.5cm,
        width=7cm,
        legend style={nodes={scale=0.8, transform shape}},
        enlarge x limits=0.05,
    ]   
    
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        % MAJORITY MINP 0.01
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        
        \addplot[ line width=1pt, blue, mark=triangle*]
            table [x=k, y=Score, col sep=comma]{figures/ablation/data/Majority_minp0.01.csv};
        \addlegendentry{Majority}

        \addplot[ line width=1pt, orange, mark=triangle*]
            table [x=k, y=Score, col sep=comma]{figures/ablation/data/Minority_minp0.01.csv};
        \addlegendentry{Minority}

        %%%%%%%%%%%%%%%%%
        
        \addplot[name path=upper, line width=1pt, draw=none]
            table [x=k, y expr=\thisrowno{1}+\thisrowno{5}, col sep=comma]{figures/ablation/data/Majority_minp0.01.csv};

        \addplot[name path=lower, line width=1pt, draw=none]
            table [x=k, y expr=\thisrowno{1}-\thisrowno{5}, col sep=comma]{figures/ablation/data/Majority_minp0.01.csv};

        \addplot[draw=none, forget plot, stack plots=y, color=blue, opacity=0.2] fill between [of=lower and upper];


        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        % MINORITY MINP 0.01
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

        
        %%%%%%%%%%%%%%%%%
        
        \addplot[name path=upper, line width=1pt, draw=none]
            table [x=k, y expr=\thisrowno{1}+\thisrowno{5}, col sep=comma]{figures/ablation/data/Minority_minp0.01.csv};

        \addplot[name path=lower, line width=1pt, draw=none]
            table [x=k, y expr=\thisrowno{1}-\thisrowno{5}, col sep=comma]{figures/ablation/data/Minority_minp0.01.csv};

        \addplot[draw=none, forget plot, stack plots=y, color=orange, opacity=0.2] fill between [of=lower and upper];

        \end{axis}
\end{tikzpicture}

==> figures/ablation/ablation_plot_groupplot.tex <==
\pgfplotsset{compat=newest, scaled x ticks=false}
\usepgfplotslibrary{groupplots}

\begin{tikzpicture}
  \begin{groupplot}[
    group style={
      group size=2 by 1,
      horizontal sep=1.5cm,
    },
    xlabel={$K$},
    ylabel={group score},
    symbolic x coords={2,4,16,32},
    ymajorgrids=true,
    xmajorgrids=true,
    grid style=dotted,
    height=4cm,
    width=5cm,
    enlarge x limits=0.05,
    ymin=0.57,
    error bars/y dir=both,
    error bars/y explicit,
    legend to name=sharedlegend,
    legend columns=2,
    legend style={
      nodes={scale=0.9, transform shape},
      /tikz/every even column/.append style={column sep=0.6cm}
    },
  ]

  % ------------------ First subplot ------------------
  \nextgroupplot[
    xlabel style={yshift=0.2em},
    xlabel={$K$},
  ]
  \addplot[
    black,
    line width=1pt,
    mark=triangle*,
    error bars/.cd,
    y dir=both,
    y explicit
  ] table [
    x=k,
    y=Score,
    y error expr=\thisrowno{4},
    col sep=comma
  ]{figures/ablation/data/Majority_minp0.01.csv};

  \addplot[
    black,
    dotted,
    line width=1pt,
    mark=square*,
    error bars/.cd,
    y dir=both,
    y explicit
  ] table [
    x=k,
    y=Score,
    y error expr=\thisrowno{4},
    col sep=comma
  ]{figures/ablation/data/Minority_minp0.01.csv};

  % ------------------ Second subplot ------------------
  \nextgroupplot[
    xlabel style={yshift=0.2em},
    xlabel={$K$},
  ]
  \addplot[
    black,
    line width=1pt,
    mark=triangle*,
    error bars/.cd,
    y dir=both,
    y explicit
  ] table [
    x=k,
    y=Score,
    y error expr=\thisrowno{4},
    col sep=comma
  ]{figures/ablation/data/Majority_minp0.2.csv};
  \addlegendentry{Majority}

  \addplot[
    black,
    dotted,
    line width=1pt,
    mark=square*,
    error bars/.cd,
    y dir=both,
    y explicit
  ] table [
    x=k,
    y=Score,
    y error expr=\thisrowno{4},
    col sep=comma
  ]{figures/ablation/data/Minority_minp0.2.csv};
  \addlegendentry{Minority}

  \end{groupplot}

  % Draw shared legend centered above the groupplot
  \node at ($(group c1r1)!.5!(group c2r1)+(0,2.3cm)$) {\ref{sharedlegend}};

\end{tikzpicture}























% \pgfplotsset{scaled x ticks=false}
% \usepgfplotslibrary{groupplots}  % for \begin{groupplot}

% \begin{tikzpicture}
%   \begin{groupplot}[
%     group style={
%       group size=2 by 1,       % 2 columns, 1 row
%       horizontal sep=1.5cm,    % space between plots
%       vertical sep=1cm,        % (won’t matter much here)
%     },
%     xlabel=Inner Dimension $k$,
%     ylabel=\texttt{Shared-Pref} $\pi_{\rm PPO}$ Avg. Score,
%     symbolic x coords={2,4,16,32},
%     legend pos=north east,
%     ymajorgrids=true,
%     xmajorgrids=true,
%     grid style=dotted,
%     height=5.5cm,
%     width=7cm,
%     legend style={nodes={scale=0.8, transform shape}},
%     enlarge x limits=0.05,
%   ]
%     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     % first subplot
%     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
%     \nextgroupplot[title={Minority Proportion: $0.01$}]
    
%     \addplot[ line width=1pt, blue, mark=triangle*]
%         table [x=k, y=Score, col sep=comma]{figures/ablation/data/Majority_minp0.01.csv};
%     %\addlegendentry{Majority}

%     \addplot[ line width=1pt, orange, mark=triangle*]
%         table [x=k, y=Score, col sep=comma]{figures/ablation/data/Minority_minp0.01.csv};
%     %\addlegendentry{Minority}

%     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     % MAJORITY MINP 0.01
%     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     \addplot[name path=upper, line width=1pt, draw=none]
%         table [x=k, y expr=\thisrowno{1}+\thisrowno{4}, col sep=comma]{figures/ablation/data/Majority_minp0.01.csv};

%     \addplot[name path=lower, line width=1pt, draw=none]
%         table [x=k, y expr=\thisrowno{1}-\thisrowno{4}, col sep=comma]{figures/ablation/data/Majority_minp0.01.csv};

%     \addplot[draw=none, forget plot, stack plots=y, color=blue, opacity=0.2] fill between [of=lower and upper];

%     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     % MINORITY MINP 0.01
%     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     \addplot[name path=upper, line width=1pt, draw=none]
%         table [x=k, y expr=\thisrowno{1}+\thisrowno{4}, col sep=comma]{figures/ablation/data/Minority_minp0.01.csv};

%     \addplot[name path=lower, line width=1pt, draw=none]
%         table [x=k, y expr=\thisrowno{1}-\thisrowno{4}, col sep=comma]{figures/ablation/data/Minority_minp0.01.csv};

%     \addplot[draw=none, forget plot, stack plots=y, color=orange, opacity=0.2] fill between [of=lower and upper];
    
%     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     % Second PLot
%     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     \nextgroupplot[title={Minority Proportion: $0.2$}]
%     \addplot[ line width=1pt, blue, mark=triangle*]
%         table [x=k, y=Score, col sep=comma]{figures/ablation/data/Majority_minp0.2.csv};
%     \addlegendentry{Majority}

%     \addplot[ line width=1pt, orange, mark=triangle*]
%         table [x=k, y=Score, col sep=comma]{figures/ablation/data/Minority_minp0.2.csv};
%     \addlegendentry{Minority}

%     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     % MAJORITY MINP 0.01
%     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     \addplot[name path=upper, line width=1pt, draw=none]
%         table [x=k, y expr=\thisrowno{1}+\thisrowno{4}, col sep=comma]{figures/ablation/data/Majority_minp0.2.csv};

%     \addplot[name path=lower, line width=1pt, draw=none]
%         table [x=k, y expr=\thisrowno{1}-\thisrowno{4}, col sep=comma]{figures/ablation/data/Majority_minp0.2.csv};

%     \addplot[draw=none, forget plot, stack plots=y, color=blue, opacity=0.2] fill between [of=lower and upper];

%     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     % MINORITY MINP 0.01
%     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     \addplot[name path=upper, line width=1pt, draw=none]
%         table [x=k, y expr=\thisrowno{1}+\thisrowno{4}, col sep=comma]{figures/ablation/data/Minority_minp0.2.csv};

%     \addplot[name path=lower, line width=1pt, draw=none]
%         table [x=k, y expr=\thisrowno{1}-\thisrowno{4}, col sep=comma]{figures/ablation/data/Minority_minp0.2.csv};

%     \addplot[draw=none, forget plot, stack plots=y, color=orange, opacity=0.2] fill between [of=lower and upper];
    
%   \end{groupplot}
% \end{tikzpicture}

==> math_commands.tex <==

\usepackage{amsmath,amsfonts,bm}

\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

\newcommand{\newterm}[1]{{\bf #1}}


\def\figref#1{figure~\ref{#1}}
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
\def\secref#1{section~\ref{#1}}
\def\Secref#1{Section~\ref{#1}}
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
\def\eqref#1{Eq.~\ref{#1}}
\def\Eqref#1{Equation~\ref{#1}}
\def\plaineqref#1{\ref{#1}}
\def\chapref#1{chapter~\ref{#1}}
\def\Chapref#1{Chapter~\ref{#1}}
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
\def\algref#1{Alg.~\ref{#1}}
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
\def\partref#1{part~\ref{#1}}
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}
\newcommand{\calO}{\cal{O}}
\def\eps{{\epsilon}}


\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

\newcommand{\pdata}{p_{\rm{data}}}
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} %

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\Ex}[1]{\ensuremath{\mathbb{E}\left[ #1 \right]}}
\newcommand{\varEx}[2]{\ensuremath{\mathbb{E}_{#1}\left[ #2 \right]}}

\newcommand{\norm}[2]{\ensuremath{{\left\| #1 \right\|}_{#2}}}
\newcommand{\normtwo}[1]{\ensuremath{{\left\| #1 \right\|}_{2}}}
\newcommand{\normf}[1]{\ensuremath{{\left\| #1 \right\|}_{F}}}
\newcommand{\normop}[1]{\ensuremath{{\left\| #1 \right\|}_{\mathrm{op}}}}
\newcommand{\normp}[1]{\ensuremath{{\| #1 \|}_{p}}}
\newcommand{\norminf}[1]{\ensuremath{{\| #1 \|}_{\infty}}}

\newcommand{\abs}[1]{\ensuremath{\vert #1 \vert}}

\renewcommand{\th}{\ensuremath{{}^{\mathrm{th}}}}

\newcommand{\parents}{Pa} %

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak



\DeclareMathOperator*{\ex}{\mathbb{E}}
\DeclareMathOperator*{\Prob}{\mathrm{Pr}}
\DeclareMathOperator{\tr}{\mathsf{tr}}
\DeclareMathOperator{\dt}{\mathsf{det}}
\DeclareMathOperator*{\dir}{\mathrm{Dir}}
\DeclareMathOperator*{\mul}{\mathrm{Mul}}
\DeclareMathOperator*{\bin}{\mathrm{Bin}}
\DeclareMathOperator*{\dirmul}{\mathrm{DirMul}}


\newcommand{\eqdef}{\mathrel{\mathop=}:}
\newcommand{\paren}[1]{\left( #1 \right)}
\newcommand{\innerprod}[2]{\langle #1, \; #2\rangle}
\newcommand{\inprod}[2]{\ensuremath{\langle {#1}, \; {#2} \rangle}}

\newcommand{\lzone}{l_{0-1}}
\newcommand{\brck}[1]{\left [ #1 \right ] }
\newcommand{\cbrck}[1]{\left \{ #1 \right \} }
\newcommand{\indicator}{\mathbbm{1}}

\renewcommand{\eps}{\varepsilon}

\renewcommand{\cal}{\mathcal}

\newcommand{\T}{\ensuremath{\top}}

\newcommand{\Zpriv}{\ensuremath{Z_{\mathrm{priv}}}}
\newcommand{\Zpub}{\ensuremath{Z_{\mathrm{pub}}}}

\newcommand{\xpriv}{\ensuremath{x_{\mathrm{priv}}}}
\newcommand{\xpub}{\ensuremath{x_{\mathrm{pub}}}}
\newcommand{\Xpriv}{\ensuremath{X_{\mathrm{priv}}}}
\newcommand{\Xpub}{\ensuremath{X_{\mathrm{pub}}}}
\newcommand{\priv}{\ensuremath{\mathrm{priv}}}
\newcommand{\pub}{\ensuremath{\mathrm{pub}}}

\newcommand{\dUnif}{\mathsf{Unif}}
\newcommand{\dBeta}{\mathsf{Beta}}
\newcommand{\dBer}{\mathsf{Ber}}

\newcommand{\bX}{\mathbf{X}}

\newcommand{\Dpriv}{\cal{D}_\priv}
\newcommand{\Dpub}{\cal{D}_\pub}
\newcommand{\data}{\cal{D}}


\newcommand{\pibase}{\pi_b}
\newcommand{\dexp}{\mathcal{D}_e}
\newcommand{\piexp}{\pi_e}
\newcommand{\kl}[2]{D_{\mathrm{KL}} \paren{#1 \| #2}}
\newcommand{\He}{\mathbbm{H}}
\newcommand{\hell}[2]{D_{\mathrm{H}^2} \paren{#1 , #2}}
\newcommand{\chisq}[2]{D_{\chi^2} \paren{#1 \| #2}}
\newcommand{\tv}[2]{D_{\mathrm{TV}} \paren{#1 , #2}}
\newcommand{\VG}{\mathrm{VG}}
\newcommand{\bs}{\mathbf{s}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\gsim}{\raisebox{-0.13cm}{~\shortstack{$>$ \\[-0.07cm] $\sim$}}~} \newcommand{\lsim}{\raisebox{-0.13cm}{~\shortstack{$<$ \\[-0.07cm] $\sim$}}~}
\newcommand{\ellzone}{\ell_{0/1}}
\newcommand{\est}{\textbf{Est}^{\text{Off}}_n}


==> multi_objective_RLHF_infancy/arch.tex <==
\section{Figures}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{figures/architecture.pdf}
    \caption{Caption}
    \label{fig:architecture}
\end{figure}
